A Study of Static Warning Cascading Tools (Experience Paper)

Static analysis is widely used for software assurance. However, static analysis tools can report an overwhelming number of warnings, many of which are false positives. Applying static analysis to a new version, a large number of warnings can be only relevant to the old version. Inspecting these warnings is a waste of time and can prevent developers from finding the new bugs in the new version. In this paper, we report the challenges of cascading warnings generated from two versions of programs. We investigated program differencing tools and extend them to perform warning cascading automatically. Specifically, we used textual based diff tool, namely SCALe, abstract syntax tree (AST) based diff tool, namely GumTree, and control flow graph (CFG) based diff tool, namely Hydrogen. We reported our experience of applying these tools and hopefully our findings can provide developers understandings of pros and cons of each approach. In our evaluation, we used 96 pairs of benchmark programs for which we know ground-truth bugs and fixes as well as 12 pairs of real-world open-source projects. Our tools and data are available at https: //github.com/WarningCas/WarningCascading_Data.

==> Algorithm/OverviewFlow.tex <==
% kjnj/po
\usetikzlibrary{positioning}
\begin{figure*}

\tikzstyle{input} = [rectangle, align=center, text centered]
\tikzstyle{block} = [rectangle, draw, align=center, text centered, minimum height = 3.0em]
\tikzstyle{output} = [rectangle, align=center, text centered]
%\resizebox{\textwidth}{
\begin{tikzpicture}[auto, every node/.append style={thick, rounded corners=2pt}]
  % \draw [help lines] (-11,-2) grid (7,2);
  \node [input] at (-10,0) (Prog) {Program Versions\\ ($V_1$, $V_2$)};
  \node [block] at (-7.5,1) (SAS) {Static Analyzer\\ Tools};
  \node [block, minimum width = 6.0em] at (-7.5,-1) (Build) {Hydrogen};
  \node [block] at (-4.5,0) (Embed) {Embed Warnings\\ in MVICFG};
  \node [block, minimum height = 5.0em] at (-1.3,0) (Match) {Match Warnings\\ in shared \\MVICFG nodes};
  \node [block, minimum height = 5.0em] at (1.9,0) (Path) {Compute Paths\\ for \\Matched Warnings};
  \node [output] at (5.6,0) (Output) {Cascaded Warnings\\ $(M_{SP}, M_{DP}, W_1,W_2)$};
  \begin{scope}[on background layer]
    \node [dashed,block,label=above:{\texttt{CascadeWarning}},minimum width=6.5cm,minimum height = 2.25cm] at (0.375,0.0cm) (bg) {};
  %you may also use align = center instead of text width = ...
  \end{scope}

  \draw[->,thick] (Prog) |- node[]  {} (SAS);
  \draw[->,thick] (Prog) |- node[]  {} (Build);
  \draw[->,thick] (SAS) -| node[near start, above]   {$SW_1$,$SW_2$} (Embed);
  \draw[->,thick] (Build) -| node[near start, below] {MVICFG} (Embed);
  \draw[->,thick] (Embed) -- node[] {} (Match);
  \draw[->,thick] (Match) -- node[] {} (Path);
  \draw[->,thick] (Path) -- node[] {} (Output);
\end{tikzpicture}
%}
	\caption{The Workflow of \toolname}
	\label{fig:flowChart}
\end{figure*}
